H-GLow: Accelerating Graph Generation via Hazard-Guided Discrete Flow Matching

Discrete flow matching (DFM) offers a promising approach to graph generation; however, generating high-quality graphs with few steps remains challenging due to the strong dependencies between nodes and edges. Although DFM decouples training from sampling, enabling flexible sampling strategies without retraining, existing graph DFM samplers often rely on task-specific heuristics, substantially expanding the hyperparameter space. Moreover, graph DFM models still require sampling budgets comparable to those of diffusion-based approaches, leaving their potential for accelerating graph generation only partially realized. In this work, we introduce H-Glow, a hazard-guided framework for accelerating graph generation built on the decomposition of Continuous-Time Markov chain (CTMC) generators into hazards and conditional jump distributions. H-Glow leverages these quantities to plan graph edits and dynamically adjust the sampling time to graph activity. H-Glow can be adapted to pretrained graph DFM models, substantially improving the generation quality with fewer steps. We further introduce a novel graph DFM model based on the conditional generator matching framework, which directly predicts hazards and conditional jumps, and show that its training objective decomposes exactly into hazard matching and hazard-weighted jump prediction. Experiments on molecular and synthetic graph benchmarks demonstrate improved generation quality with substantially fewer sampling steps.

==> algorithms/adaptive_hazard_clock_sampler.tex <==
\todo{Adjust either based on HGlow training or Using a pretrained model.}
\begin{wrapfigure}{r}{0.52\textwidth}
\vspace{-2\baselineskip}
\centering
\begin{minipage}{\linewidth}
\begin{algorithm}[H]
\caption{Hazard-Guided Sampling with \ours{}}
\label{alg:hglow-sampling}
\begin{algorithmic}[1]
\State \textbf{Input:} model $f_\theta$, steps $T$
\State Sample $G_0\sim p_0$ and set $t\gets 0$

\For{$k=1,\ldots,T$}
    \If{$t\geq t_{\mathrm{stop}}$}
        \State \textbf{break} 
        %\Comment{Early stopping}
    \EndIf

    \State
    $(\boldsymbol{\hazard}_{\theta,t}^{X},
    \boldsymbol{\jump}_{\theta,t}^{X},
    \boldsymbol{\hazard}_{\theta,t}^{E},
    \boldsymbol{\jump}_{\theta,t}^{E})
    \gets f_\theta(G_t,t)$ 
    %\\ \Comment{Predict hazards and jumps}

    \State
    $T_{\theta,t}(G_t)
    \gets
    w_X\sum_i\hazard_{\theta,t}^{X,i}
    +
    \sum_{i<j}\hazard_{\theta,t}^{E,ij}$
    %\Comment{Compute total hazard}

    \State
    $\Delta t
    \gets
    \min\!\left\{
        1/T_{\theta,t}(G_t),\,1-t
    \right\}$
    %\Comment{Adaptive time jump}

    \State
    $c\sim\Cat\!\left(
        \{w_X\hazard_{\theta,t}^{X,i}\}_{i=1}^{N}
        \cup
        \{\hazard_{\theta,t}^{E,ij}\}_{i<j}
    \right)$
    %\Comment{Select component}

    \State Sample
    $\tilde z\sim{\jump}_{\theta,t}^{(c)}$
    and update component $c$ in the graph
    %\Comment{Sample jump}

    \State $t\gets t+\Delta t$
\EndFor

\State \Return $G_1$
\end{algorithmic}
\end{algorithm}
\end{minipage}
\vspace{-2\baselineskip}
\end{wrapfigure}

==> algorithms/adaptive_tau_leaping.tex <==
\newpage
\begin{algorithm}[H]
\caption{One-Clock Hazard-Guided Sampling with \ours{}}
\label{alg:hglow-oneclock-sampling}
\begin{algorithmic}[1]
\State \textbf{Input:} model $f_\theta$, number of steps $T$
\State Sample $G\sim p_0$ and set $t\gets t_{\min}$
%\State $\mathcal C_X\gets\{i\}_{i=1}^{N}$,        $\mathcal C_E\gets\{(i,j):i<j\}$
%\State $\mathcal C\gets\mathcal C_X\cup\mathcal C_E$
%\State $\omega_c\gets w_X$ for $c\in\mathcal C_X$,      and $\omega_c\gets 1$ for $c\in\mathcal C_E$

\For{$k=1,\ldots,T$}
    \State
    $(\boldsymbol{\hazard}_{\theta,t}^{X},
      \boldsymbol{\jump}_{\theta,t}^{X},
      \boldsymbol{\hazard}_{\theta,t}^{E},
      \boldsymbol{\jump}_{\theta,t}^{E})
    \gets f_\theta(G,t)$

    \State $a_{\theta,t}^{(c)}
        \gets (1-t)\hazard_{\theta,t}^{(c)}
        \quad \forall c\in\mathcal C$

    \State $\bar a_{\theta,t}\gets
        \frac12\left(
        \frac{\sum_i a_{\theta,t}^{X,i}}{N}
        +
        \frac{\sum_{i<j}a_{\theta,t}^{E,ij}}
             {\max\{1,\binom{N}{2}\}}
        \right)$

    \State $\widehat t\gets
        \operatorname{clip}
        (1-\bar a_{\theta,t},t_{\min},t_{\max})$

    \State $T_{\theta,t}(G)\gets
        w_X\sum_i\hazard_{\theta,t}^{X,i}
        +\sum_{i<j}\hazard_{\theta,t}^{E,ij}$

    \If{$T_{\theta,t}(G)\leq 10^{-12}$}
        \State \Return $G$
    \EndIf

    \State $\Delta t\gets
        \min\!\left\{
            \max\!\left\{
                \frac{1}{T_{\theta,t}(G)},
                \frac{t_{\max}-t}{T-k}
            \right\},
            t_{\max}-t
        \right\}$

    \State $\widetilde G\gets G$
    \ForAll{$c\in\mathcal C$}
        \State $p_c\gets
            1-\exp\!\left(
                -s\,\omega_c\,a_{\theta,t}^{(c)}\,\Delta t
            \right)$
        \State $b_c\sim\operatorname{Bernoulli}(p_c)$
            %wa\Comment{Independently}
        \If{$b_c=1$}
            \State $\widetilde G^{(c)}
                \sim\Cat(\jump_{\theta,t}^{(c)})$
        \EndIf
    \EndFor
    %\State $G\gets\widetilde G$; restore edge symmetry
    \State $t\gets\widehat t$
        \Comment{One-clock update}
\EndFor
\State \Return $G$
\end{algorithmic}
\end{algorithm}

==> algorithms/gillepsie_sampler.tex <==
\begin{algorithm}[t]
\caption{Adaptive Exit-Hazard Clock Sampling}
\label{alg:adaptive-clock}
\begin{algorithmic}[1]
\Require
    trained decomposed model $p_\theta$;
    NFE budget $T$;
    edits per NFE $m$;
    initial clock $\kappa_{\min}$;
    stopping target $\kappa_{\max}$;
    node weight $w_X$;
    hazard power $\gamma$;
    confidence power $\rho$;
    jump temperature $\tau$.
\State Sample an initial graph
       $G=(X,E)$ from the source distribution.
\State Initialize the model clock
       $\kappa \gets \kappa_{\min}$.
\For{$s=1,\ldots,T$}
    \State Predict decomposed exit probabilities and jump distributions:
    \[
    \{q_i^X,J_i^X\}_{i\in V},
    \quad
    \{q_{ij}^E,J_{ij}^E\}_{(i,j)\in\mathcal E}
    \gets p_\theta(G,\kappa).
    \]
    \State Compute the mean node and edge exit masses:
    \[
    \bar q_X
      \gets \frac{1}{|V|}\sum_{i\in V}q_i^X,
    \qquad
    \bar q_E
      \gets \frac{1}{|\mathcal E|}
             \sum_{i<j}q_{ij}^E.
    \]
    \State Infer the graph's current clean-time coordinate:
    \[
    \widehat{\kappa}
      \gets
      \operatorname{clip}\!\left(
        1-\frac{\bar q_X+\bar q_E}{2},
        \kappa_{\min},
        \kappa_{\max}
      \right).
    \]
    \State Update the model clock:
    $\kappa\gets\widehat{\kappa}$.
    \If{$\widehat{\kappa}\geq\kappa_{\max}$}
        \State Continue without editing $G$.
        \Comment{Per-sample early stopping}
    \EndIf
    \State Apply jump temperature:
    \[
    \widetilde J_c(a)
      \gets
      \frac{J_c(a)^{1/\tau}}
           {\sum_b J_c(b)^{1/\tau}}
    \quad\text{for every component }c.
    \]
    \State Construct global component-selection weights:
    \[
    h_i^X
      \gets w_X q_i^X
             \left(\max_a\widetilde J_i^X(a)\right)^\rho,
    \]
    \[
    h_{ij}^E
      \gets q_{ij}^E
             \left(\max_a\widetilde J_{ij}^E(a)\right)^\rho.
    \]
    \State Apply hazard sharpening:
    \[
    \omega_c \gets h_c^\gamma.
    \]
    \For{$r=1,\ldots,m$}
        \State Select a component without replacement:
        \[
        c\sim\operatorname{Categorical}
        \left(
          \frac{\omega_c}{\sum_{c'}\omega_{c'}}
        \right).
        \]
        \State Sample its new categorical state:
        \[
        z_c'
        \sim\operatorname{Categorical}
        \bigl(\widetilde J_c\bigr).
        \]
        \State Set $z_c\gets z_c'$.
        \If{$c$ is an edge $(i,j)$}
            \State Enforce symmetry:
            $E_{ji}\gets E_{ij}$.
        \EndIf
        \State Set $\omega_c\gets 0$.
        \Comment{Do not select the same component twice}
    \EndFor
\EndFor
\State \Return the final graph $G=(X,E)$.
\end{algorithmic}
\end{algorithm}

==> algorithms/hglow_set_update.tex <==
\begin{algorithm}[t]
\caption{\ours{}: Hazard-guided set sampling}
\label{alg:hazard-set-sampling}
\begin{algorithmic}[1]
\State \textbf{Input:} model $f_\theta$, NFE budget $T$,
update budget $B$, threshold $T_{\mathrm{stop}}$
\State Sample $G_0\sim p_0$ and set $t_0\gets 0$, $k\gets 0$
\State Let $\mathcal C=\mathcal C_X\cup\mathcal C_E$

\While{$k<T$}
    \State Construct component generators
    $\{R_{\theta,t_k}^c\}_{c\in\mathcal C}$ from $(G_k,t_k)$

    \State Decompose the generators:
    $
    \left\{
    \hazard_{\theta,t_k}^c,
    \jump_{\theta,t_k}^c
    \right\}_{c\in\mathcal C}
    $

    \State
    $
    T_{\theta,t_k}
    \gets
    \sum_{c\in\mathcal C}
    \hazard_{\theta,t_k}^c
    $

    \If{$T_{\theta,t_k}<T_{\mathrm{stop}}$}
        \State \Return $G_k$
    \EndIf

    \State 
    $
    \overline{\hazard}_{\theta,t_k}^{X}
    \gets
    \frac{1}{N}
    \sum_{c\in\mathcal C_X}
    \hazard_{\theta,t_k}^c,
    \qquad
    \overline{\hazard}_{\theta,t_k}^{E}
    \gets
    \frac{1}{\binom{N}{2}}
    \sum_{c\in\mathcal C_E}
    \hazard_{\theta,t_k}^c
    $

    \State 
    $
    \widehat t_{k+1}
    \gets
    1-\frac{1-t_k}{2}
    \left(
    \overline{\hazard}_{\theta,t_k}^{X}
    +
    \overline{\hazard}_{\theta,t_k}^{E}
    \right)
    $

    \State Set
    $
    t_{k+1}
    \gets
    \operatorname{clip}
    \left(\widehat t_{k+1},0,1-\varepsilon\right)
    $

    \State Set the leap size
    $
    \Delta_k
    \gets
    \frac{B}{T_{\theta,t_k}+\varepsilon}
    $

    \ForAll{$c\in\mathcal C$}
        \State Compute the selection probability
        $
        q_k^c
        \gets
        1-\exp\left(
        -\Delta_k\hazard_{\theta,t_k}^c
        \right)
        $

        \State Sample
        $
        b_k^c\sim\operatorname{Bernoulli}(q_k^c)
        $
    \EndFor

    \State Select the update set
    $
    \mathcal S_k
    \gets
    \left\{
    c\in\mathcal C:b_k^c=1
    \right\}
    $
    %\If{$\mathcal S_k=$}
    %    \State Sample
    %    $
    %    c_k\sim
     %    \operatorname{Cat}
     %    \left(
     %    \left\{
     %    \frac{\hazard_{\theta,t_k}^c}
     %         {T_{\theta,t_k}}
     %    \right\}_{c\in\mathcal C}
     %    \right)
     %    $
      %   \State Set $\mathcal S_k\gets\{c_k\}$
     %\EndIf

    \ForAll{$c\in\mathcal S_k$}
        \State Sample
        $
        \widetilde z_k^c
        \sim
        \jump_{\theta,t_k}^c
        $
    \EndFor

    \State 
    $
    G_{k+1}
    \gets
    \operatorname{Update}
    \left(
    G_k,
    \left\{
    (c,\widetilde z_k^c)
    \right\}_{c\in\mathcal S_k}
    \right)$
    

    \State $k\gets k+1$
\EndWhile

\State \Return $G_k$
\end{algorithmic}
\end{algorithm}

==> chapters/introduction.tex <==
%\section{Introduction}

%Motivation:
%\begin{itemize}
%    \item A permutation-equivariant graph-edit jump process with directly learned structural hazards, together with a graph-specific hazard controller that handles parallel edits, conflicts, constraints, and adaptive computation.
%    \item Two states with similar clean posteriors can have different predicted exit intensities.
%    \item **Event-Factorized RVF denoiser** Standard RVF denoisers conflate event occurrence and event destination in one categorical prediction. We explicitly expose these two quantities, enabling independently calibrated activity prediction and event-based low-NFE sampling while preserving a valid, clean posterior.
%    \item Direct event allocation $$ \frac{\lambda_i}{\sum_j\lambda_j} $$ explicitly ranks which components should receive the NFE budget.
%    \item The CTMC objective is more directly aligned with rate accuracy; CE is aligned with endpoint classification.
%    \item We replace SimGFM’s endpoint-induced, tightly coupled rate with directly learned node- and edge-level exit and jump dynamics, enabling explicit activity calibration and low-NFE hazard-controlled parallel sampling.
%    \item We want to avoid over/under editing the graph during sampling, which can lead to decreased performance.
%    \item Model training: hazard-aware?: decompose to when to jump, where to jump: $A_t$ controls the correction budget; $\pi_t$ controls which node or edge is reconsidered; $r_t(\cdot \mid \cdot)$ controls the replacement node or edge category.
%    \item Sampler: avoid over/under editing.

%    \item "Clean-label CE directly optimizes neither the total graph hazard nor the event count. It can learn them implicitly through the clean posterior, but it does not explicitly isolate their calibration." Can we somehow show this? "DisCo and Cometh train clean-graph predictors and obtain reverse transition rates only through a subsequent forward-kernel-dependent transformation. Consequently, total event intensity, component selection, and jump destination are coupled implicitly within a single denoising posterior. We instead directly parameterize the graph reverse generator as total activity, component allocation, and conditional jump distribution. This hierarchical parameterization mirrors the global CTMC event mechanism and induces an exact decomposition of the path-space objective into losses for event intensity, event location, and event type. It therefore enables direct calibration and control of graph-edit dynamics and naturally supports global event-based and adaptive samplers."
%\end{itemize}

%Contribution:
%\begin{itemize}
%    \item \textbf{Graph Flow Matching.} We introduce \textit{HG-DFM}, a novel HG-DFM: Hazard-Guided Discrete Flow Matching for Graph Generation. A permutation-equivariant reverse CTMC in which each legal graph edit is represented by a learned exit hazard and a conditional edit mark. 
%    \item \textbf{Graph ELBO.} A tractable graph-local rate-matching objective that decomposes into: x and y.
%    \item \textbf{Novel hazard-controlled graph sampler.} We leverage the decomposition and use the learned hazard to control sampling by adaptively discretizing the time and selecting the node/edge to update, then use the learned jump to change the selected component.  Explicit self-correction: A non-absorbing process can insert an edge, later delete it, and then insert a different edge. Learned exit hazards provide a direct way to decide which existing decisions remain unstable. Compute allocation: Low-hazard portions of the graph can be skipped, while high-hazard regions receive more event updates. This is especially attractive when only a small subgraph needs correction late in generation.
%    \item \textbf{Empirical performance.} 
    %\item Novel graph generation method. The decomposition exposes activity, allocation, and local jumps as separately measurable and controllable quantities. The decomposition is exactly a marked point process: A is the ground intensity, pi the component mark, and r the destination mark.
    %\item Why? Can accelerate graph sampling?: avoid over/under editing. TBD: Discuss issues with current CTMC samplers. But we can sample exact CTMC path
    %\item Can be applied to a pretrained model, or can we do new guidance? Or, is the stochasticty in DeFoG hurthful?
    %\item A learned noise schedule. The model effectively learns a state-dependent clock instead of inheriting all timing behavior from the forward process. The important catch is that flexibility and correctness are separate.
%\end{itemize}

\section{Introduction}

Diffusion models have emerged as a powerful approach to graph generation, achieving strong performance on molecular and synthetic graph benchmarks~\citep{GRAPH_DIFFUSION}. These models learn to reverse a gradual corruption of node and edge attributes, generating graphs through iterative denoising. 
Recent work has further introduced discrete flow matching (DFM) for graphs, formulating generation as a continuous-time Markov chain (CTMC) that transports a simple prior distribution toward the data distribution~\citep{DISCRETE_FLOW_MATCHING,GRAPH_DFM}. 
By decoupling learning from the choice of sampling dynamics, this formulation offers flexibility to improve generation at inference time without retraining.

Existing graph DFMs typically train denoising networks to predict clean node and edge attributes and use these predictions to construct the CTMC generator governing sampling~\citep{GRAPH_DFM}. 
Graphs are then generated through finite-step approximations, such as $\tau$-leaping or independent Euler updates~\citep{CTMC_SAMPLING}. 
Additional sampling heuristics, including stochasticity and target guidance, can improve sample quality but introduce further hyperparameters and design choices~\citep{SAMPLING_HEURISTICS}. 
Sampling-time schedules are also designed to concentrate computation in particular regions of the generation trajectory, with configurations depending on the dataset and sampling budget~\citep{GRAPH_SAMPLING_SCHEDULES}.
Despite progress in reducing sampling steps, realizing the acceleration potential of graph DFM across tasks and budgets remains challenging. 
In particular, coarse parallel updates use rates evaluated on the same graph to modify several components simultaneously, without accounting for interactions between these changes. 
For strongly interdependent node and edge attributes, such updates can compromise structural or chemical validity. This motivates sampling strategies that coordinate graph edits and adapt computation to the evolving graph.

In this work, we introduce \ours{}, a novel hazard-guided sampler for graph generation built on the decomposition of CTMC generators into exit hazards and conditional jump distributions. 
Hazards quantify the instantaneous propensity of each node or edge to change, while conditional jumps specify its destination attribute. \ours{} uses these quantities to plan graph edits and leverages model-predicted activity to jointly determine which graph components change, what conditioning time to use next, and when to terminate generation. Combining hazards with jump confidence prioritizes component updates, while a dynamic, hazard-guided schedule adapts model-query times to the current graph. Early stopping further avoids unnecessary edits when the predicted activity becomes low. For molecular generation, recomputing predictions after each selected edit allows subsequent updates to account for the modified graph, reducing reliance on simultaneous decisions made from an unchanged state. We also introduce a parallel extension for graphs requiring more edits within a limited evaluation budget.

The modular nature of this construction allows \ours{} to serve as a drop-in sampler for compatible pretrained graph DFMs. Hazards and conditional jumps are extracted directly from their generators, enabling improvements in generation quality and efficiency without retraining or additional learned components. The resulting sampler uses existing model predictions to guide graph edits and sampling times, providing a model-driven alternative to manually specifying sampling-time distortions for different tasks and budgets.

Motivated by the effectiveness of hazard-guided sampling on pretrained models, we further introduce a structured DFM model tailored to graphs. Inspired by Neural CTMC~\citep{NEURAL_CTMC}, we adapt its explicit hazard--jump parameterization to categorical node and edge attributes using a permutation-equivariant graph network. We construct this graph model from the perspective of conditional generator matching~\citep{GENERATOR_MATCHING}, defining conditional target generators along a probability path connecting empirical node and edge priors to clean graphs. 
Under the hazard--jump decomposition, we show that the graph generator matching objective separates exactly into a Poisson divergence for hazard matching and a hazard-weighted categorical KL divergence for conditional jump prediction. 
The resulting formulation directly learns the quantities used by the sampler to coordinate graph edits and allocate computation.

Extensive experiments on molecular and synthetic graph benchmarks demonstrate the effectiveness of \ours{} under limited sampling budgets. On QM9, MOSES, and GuacaMol~\citep{MOLECULAR_BENCHMARKS}, \ours{} achieves state-of-the-art FCD among the evaluated methods using 50, 100, and 100 sampling steps, respectively, outperforming the corresponding 500-step baselines. Applied to pretrained DeFoG~\citep{DEFOG}, our sampler matches or exceeds its 500-step base sampler in validity and FCD using only 100 steps, without retraining. 
Strong results on planar and tree graphs~\citep{SYNTHETIC_BENCHMARKS} further demonstrate its applicability beyond molecular generation.

We summarize our contributions as follows:
\begin{itemize}
    \item We propose \ours{}, a hazard-guided sampler that uses componentwise hazards and conditional jumps to coordinate graph edits, dynamically adapt conditioning times, and terminate generation. It applies directly to compatible pretrained graph DFMs without retraining.

    \item We adapt the explicit hazard--jump parameterization to graph DFM and construct its training objective through conditional generator matching, showing an exact decomposition into hazard matching and hazard-weighted conditional jump prediction.

    \item We demonstrate strong molecular and synthetic graph generation with few sampling steps, achieving the best molecular FCD among the evaluated methods and accelerating pretrained models. Controlled sampler comparisons and ablations support the effectiveness of our design.
\end{itemize}

==> tables/full_table.tex <==
\todo{GuacaMol: We convert samples to charged molecules following prior works, then evaluate.}

\begin{table}[t]
\centering
\caption{Large molecule generation performance on GuacaMol and MOSES.
Best scores are shown in \textbf{bold}, and second-best scores are
\underline{underlined}.}
\label{tab:large_molecule_gen}

\resizebox{\textwidth}{!}{%
\begin{tabular}{lcc*{5}{c}|*{7}{c}}
\toprule
& & & \multicolumn{5}{c}{GuacaMol}
& \multicolumn{7}{c}{MOSES} \\
\cmidrule(lr){4-8}\cmidrule(lr){9-15}

Model & Class & \# Steps
& Val.\,$\uparrow$
& V.U.\,$\uparrow$
& V.U.N.\,$\uparrow$
& KL div.\,$\uparrow$
& FCD\,$\uparrow$
& Val.\,$\uparrow$
& Unique.\,$\uparrow$
& Novelty\,$\uparrow$
& Filters\,$\uparrow$
& FCD\,$\downarrow$
& SNN\,$\uparrow$
& Scaf.\,$\uparrow$ \\
\midrule

Training set
& --
& --
& 100.0 & 100.0 & 0.0 & 99.9 & 92.8
& 100.0 & 100.0 & 0.0 & 100.0 & 0.01 & 0.64 & 99.1 \\

\midrule

DiGress{\tiny~\citep{vignac2022digress}}
& \small{Diffusion}
& 500
& 85.2 & 85.2 & 85.1 & 92.9 & 68.0
& 85.7 & \textbf{100.0} & 95.0 & 97.1 & 1.19 & 0.52 & 14.8 \\

%DisCo{\tiny~\citep{xu2024discrete}}
%& \small{Diffusion}
%& 50
%& 85.9 & 85.9 & 85.2 & 94.2 & 82.7
%& 86.8 & 100.0 & 93.1 & 97.7 & 0.95 & 0.6 & 15.2 
%\\

%DisCo{\tiny~\citep{xu2024discrete}}
%& \small{Diffusion}
%& 100
%& 87.0 & 87.0 & 86.3 & 94.6 & 82.9
%& 87.2 & 100.0 & 92.3 & 98.3 & 0.94 & 0.6 & 12.9
%\\

%DisCo{\tiny~\citep{xu2024discrete}}
%& \small{Diffusion}
%& 200
%& {88.1} & {88.1} & {87.4}& {94.9} & {83.3}
%& 87.5 & 100.0 & 92.3 & 98.5 & 1.00 & 0.6 & 13.6
%\\

DisCo{\tiny~\citep{xu2024discrete}}
& \small{Diffusion}
& 500
& 86.6 & 86.6 & 86.5 & 92.6 & 59.7
& 88.3 & \textbf{100.0} & \textbf{97.7} & 95.6 & 1.44 & 0.50 & 15.1
\\

%Cometh{\tiny~\citep{siraudin2024cometh}}
%& \small{Diffusion}
%& 50
%& 89.3 & 89.2 & 88.4 & 92.9 & 68.2
%& 82.5 & 100.0 & 97.0 & 95.2 & 1.2 & 0.5 & 16. \\

%Cometh{\tiny~\citep{siraudin2024cometh}}
%& \small{Diffusion}
%& 100
%& 93.5 & 93.4 & 92.8 & 93.9 & 72.5
%& 84.7 & 100.0 & 96.5 & 96.6 & 1.2 & 0.5 & 17.6\\

%Cometh{\tiny~\citep{siraudin2024cometh}}
%& \small{Diffusion}
%& 200
%& 94.8 & 94.8 & 93.9 & 94.1 & 74.3
%& 85.9 & 100.0 & 96.2 & 97.4 & 1.1 & 0.5 & 14.6 %\\

Cometh{\tiny~\citep{siraudin2024cometh}}
& \small{Diffusion}
& 500
& 94.4 & 94.4 & 93.5 & 94.1& 67.4
& 86.1 & 100.0 & 96.0 & 97.3 & 1.2 & 0.5 & 16.4\\

Cometh-PC{\tiny~\citep{siraudin2024cometh}}
& \small{Diffusion}
& 500
& 98.9 & 98.9 & 97.6 & 96.7 & 72.7
& 90.5 & \underline{99.9} & 92.6 & 99.1 & 1.27 & 0.54 & 16.0 \\

%IDDM{\tiny~\citep{kollovieh2026interpolating}}
%& \small{Diffusion}
%& 500
%& \textbf{99.6} & \textbf{99.5} & 97.8 & -- & 78.3
%& 90.7 & \underline{99.9} & 90.2 & 99.4 & 1.58 & 0.56 & 13.2 \\

%SimGFM{\tiny~\citep{luosimgfm}}
%& \small{Flow}
%& 50
%& 98.9 & 98.9 & 98.3 & 93.6 & 79.6
%& 86.1 & \textbf{100.0} & \underline{97.5} & 95.3 & 1.44 & 0.51 & 16.9 \\

%SimGFM{\tiny~\citep{luosimgfm}}
%& \small{Flow}
%& 200
%& \underline{99.2} & \underline{99.2} & \textbf{98.8} & 94.0 & \textbf{80.8}
%& 89.4 & \textbf{100.0} & 94.6 & 98.9 & \textbf{1.08} & 0.55
%& \underline{17.3} \\

SimGFM{\tiny~\citep{luosimgfm}}
& \small{Flow}
& 500
& \underline{99.2} & \underline{99.2} & \underline{98.6} & 94.6
& \underline{79.7}
& 91.1 & \textbf{100.0} & 93.5 & 99.2 & 1.19 & 0.56 & 14.4 \\

\midrule

%DeFoG{\tiny~\citep{qin2025defog}}
%& \small{Flow}
%& 50
%&91.7 &91.7 &91.2 &92.3 &57.9 &83.9 &99.9 &96.9 &96.5 &1.87 &0.50 &23.5 \\

%DeFoG{\tiny~\citep{qin2025defog}}
%& \small{Flow}
%& 500
%&99.0 &99.0 &97.9 &97.7 &73.8 &92.8 &99.9 &92.1 &98.9 &1.95 &0.55 &14.4 \\
%\midrule

DeFoG{\tiny~\citep{qin2025defog}}
& \small{Flow}
& 50
& 88.2 & 88.2 & 87.5 & 92.6 & 60.1
& 82.9 & \underline{99.9} & 95.1 & 97.8 & 1.47 & 0.53
& \textbf{19.8} \\

%DeFoG{\tiny~\citep{qin2025defog}}
%& \small{Flow}
%& 100
%& 96.7 & 96.7 & 95.7 & 96.0 & 74.2
%& 88.5 & \underline{99.9} & 90.7 & 99.2 & 1.25 & \underline{0.58}
%& 16.7 \\

%DeFoG{\tiny~\citep{qin2025defog}}
%& \small{Flow}
%& 200
%& 98.0 & 98.0 & 96.9 & \textbf{98.3} & 70.1
%& 90.9 & \underline{99.9} & 89.7 & 99.3 & 1.37 & \underline{0.58}
%& 11.9 \\

DeFoG{\tiny~\citep{qin2025defog}}
& \small{Flow}
& 500
& 98.6 & 98.6 & 97.5 & \underline{97.6} & 72.5
& \textbf{91.5} & \underline{99.9} & 90.0 & 99.2 & 1.39
& \textbf{0.55} & 11.5 \\

%\midrule

%\rowcolor{gray!15}
%\textbf{\ours{}-{DeFoG}(Ours)}
%& \small{Flow}
%& 50
%& 90.8 & 90.7& 89.3& 93.3&  72.7
%& 86.7 & \underline{99.9} & 92.0 & 98.3 & 2.04 & %0.57 & 10.2 \\

%\rowcolor{gray!15}
%\textbf{\ours{}-{DeFoG} (Ours)}
%& \small{Flow}
%& 100
%& 97.9 & 97.9 & 96.3 & 97.0 & 72.4
%& 90.7 & \underline{99.9} & 92.1 & 99.1 & 1.57 & 0.57 & 15.3 \\

%\rowcolor{gray!15}
%\textbf{\ours{}-{DeFoG} (Ours)}
%& \small{Flow}
%& 200
%& 99.0 & 99.0 & 97.2 & 97.1 & 70.1
%& \underline{91.2} & \underline{99.9} & 92.1 & 99.2 & 1.39 & 0.57
%& 15.1 \\

%\rowcolor{gray!15}
%\textbf{\ours{}-{DeFoG} (Ours)}
%& \small{Flow}
%& 500
%& 99.3 &	99.2 &	97.0& 97.9&	66.8&	
%91.0 & 100.0&	92.0  &	99.3  &	1.38 &	0.57 &	15.7
%\\

\midrule

\rowcolor{gray!15}
\textbf{\ours{} (Ours)}
& \small{Flow}
& 50
& 93.4 & 93.4 & 92.8 & 90.9 & 69.6
& 88.6 & \underline{99.9} & 94.1 & 99.1 & 1.11 & 0.55 & 17.1 \\

\rowcolor{gray!15}
\textbf{\ours{} (Ours)}
& \small{Flow}
& 100
& 98.2 & 98.2 & 97.0 & 96.7 & 73.0
& 90.2 & \underline{99.9} & 92.8 & \underline{99.5}
& \underline{1.10} & \underline{0.58} & 12.4 \\

\rowcolor{gray!15}
\textbf{\ours{} (Ours)}
& \small{Flow}
& 200
& 99.3 & 99.3 & 97.9 & 96.7 & 73.4
& 91.1 & \underline{99.9} & 90.3 & \textbf{99.6}
& 1.36 & 0.57 & 13.8 \\

\rowcolor{gray!15}
\textbf{\ours{} (Ours)}
& \small{Flow}
& 500
& 99.2 & 99.2  &	97.9  &	96.8  &	73.4
& 91.5 & 100.0 & 90.0 & 99.2 & 0.12 & 0.59 & 11.5 \\
\bottomrule
\end{tabular}
}
\end{table}


==> tables/k-budget-hglow.tex <==
\begin{table}[t]
\centering
\caption{\textcolor{red}{K updates per NFE} Large molecule generation performance on GuacaMol and MOSES.
Best scores are shown in \textbf{bold}, and second-best scores are
\underline{underlined}.}
\label{tab:large_molecule_gen}

\resizebox{\textwidth}{!}{%
\begin{tabular}{lcc*{5}{c}|*{7}{c}}
\toprule
& & & \multicolumn{5}{c}{GuacaMol}
& \multicolumn{7}{c}{MOSES} \\
\cmidrule(lr){4-8}\cmidrule(lr){9-15}

Model & Class & \# Steps
& Val.\,$\uparrow$
& V.U.\,$\uparrow$
& V.U.N.\,$\uparrow$
& KL div.\,$\uparrow$
& FCD\,$\uparrow$
& Val.\,$\uparrow$
& Unique.\,$\uparrow$
& Novelty\,$\uparrow$
& Filters\,$\uparrow$
& FCD\,$\downarrow$
& SNN\,$\uparrow$
& Scaf.\,$\uparrow$ \\
\midrule

Training set
& --
& --
& 100.0 & 100.0 & 0.0 & 99.9 & 92.8
& 100.0 & 100.0 & 0.0 & 100.0 & 0.01 & 0.64 & 99.1 \\

\midrule

DiGress{\tiny~\citep{vignac2022digress}}
& \small{Diffusion}
& 500
& 85.2 & 85.2 & 85.1 & 92.9 & 68.0
& 85.7 & \textbf{100.0} & 95.0 & 97.1 & 1.19 & 0.52 & 14.8 \\

%DisCo{\tiny~\citep{xu2024discrete}}
%& \small{Diffusion}
%& 50
%& 85.9 & 85.9 & 85.2 & 94.2 & 82.7
%& 86.8 & 100.0 & 93.1 & 97.7 & 0.95 & 0.6 & 15.2 
%\\

%DisCo{\tiny~\citep{xu2024discrete}}
%& \small{Diffusion}
%& 100
%& 87.0 & 87.0 & 86.3 & 94.6 & 82.9
%& 87.2 & 100.0 & 92.3 & 98.3 & 0.94 & 0.6 & 12.9
%\\

%DisCo{\tiny~\citep{xu2024discrete}}
%& \small{Diffusion}
%& 200
%& 88.1 & 88.1 & 87.4 & 94.9 & 83.3
%& 87.5 & 100.0 & 92.3 & 98.5 & 1.00 & 0.6 & 13.6
%\\

DisCo{\tiny~\citep{xu2024discrete}}
& \small{Diffusion}
& 500
& 86.6 & 86.6 & 86.5 & 92.6 & 59.7
& 88.3 & \textbf{100.0} & \textbf{97.7} & 95.6 & 1.44 & 0.50 & 15.1 \\

%Cometh{\tiny~\citep{siraudin2024cometh}}
%& \small{Diffusion}
%& 50
%& 89.3 & 89.2 & 88.4 & 92.9 & 68.2
%& 82.5 & 100.0 & 97.0 & 95.2 & 1.2 & 0.5 & 16.0 \\

%Cometh{\tiny~\citep{siraudin2024cometh}}
%& \small{Diffusion}
%& 100
%& 93.5 & 93.4 & 92.8 & 93.9 & 72.5
%& 84.7 & 100.0 & 96.5 & 96.6 & 1.2 & 0.5 & 17.6 \\

%Cometh{\tiny~\citep{siraudin2024cometh}}
%& \small{Diffusion}
%& 200
%& 94.8 & 94.8 & 93.9 & 94.1 & 74.3
%& 85.9 & 100.0 & 96.2 & 97.4 & 1.1 & 0.5 & 14.6
%\\

Cometh{\tiny~\citep{siraudin2024cometh}}
& \small{Diffusion}
& 500
& 94.4 & 94.4 & 93.5 & 94.1 & 67.4
& 86.1 & \textbf{100.0} & \underline{96.0} & 97.3
& 1.27 & 0.5 & 16.4 \\

Cometh-PC{\tiny~\citep{siraudin2024cometh}}
& \small{Diffusion}
& 500
& \underline{98.9} & \underline{98.9} & \underline{97.6}
& 96.7 & 72.7
& 90.5 & \underline{99.9} & 92.6 & 99.1
& 1.27 & 0.54 & 16.0 \\

%IDDM{\tiny~\citep{kollovieh2026interpolating}}
%& \small{Diffusion}
%& 500
%& 99.6 & 99.5 & 97.8 & -- & 78.3
%& 90.7 & 99.9 & 90.2 & 99.4 & 1.58 & 0.56 & 13.2 \\

%SimGFM{\tiny~\citep{luosimgfm}}
%& \small{Flow}
%& 50
%& 98.9 & 98.9 & 98.3 & 93.6 & 79.6
%& 86.1 & 100.0 & 97.5 & 95.3 & 1.44 & 0.51 & 16.9 \\

%SimGFM{\tiny~\citep{luosimgfm}}
%& \small{Flow}
%& 200
%& 99.2 & 99.2 & 98.8 & 94.0 & 80.8
%& 89.4 & 100.0 & 94.6 & 98.9 & 1.08 & 0.55 & 17.3 \\

%SimGFM{\tiny~\citep{luosimgfm}}
%& \small{Flow}
%& 500
%& 99.2 & 99.2 & 98.6 & 94.6 & 79.7
%& 91.1 & 100.0 & 93.5 & 99.2 & 1.19 & 0.56 & 14.4 \\

\midrule

%DeFoG{\tiny~\citep{qin2025defog}}
%& \small{Flow}
%& 50
%& 91.7 & 91.7 & 91.2 & 92.3 & 57.9
%& 83.9 & 99.9 & 96.9 & 96.5 & 1.87 & 0.50 & 23.5 \\

%DeFoG{\tiny~\citep{qin2025defog}}
%& \small{Flow}
%& 500
%& 99.0 & 99.0 & 97.9 & 97.7 & 73.8
%& 92.8 & 99.9 & 92.1 & 98.9 & 1.95 & 0.55 & 14.4 \\

DeFoG{\tiny~\citep{qin2025defog}} $(\eta=0,\omega=0)$
& \small{Flow}
& 50
& 84.2 & 84.2 & 83.8 & 91.0 & 32.7
& 88.7 & 100.0 & 95.9 & 98.0 & 3.49 & 0.534 & 11.8 \\

DeFoG{\tiny~\citep{qin2025defog}} $(\eta=0,\omega=0)$
& \small{Flow}
& 100
& 92.3 & 92.3 & 91.8 & 92.9 & 51.4
& 89.5 & 100.0 & 95.6 & 98.2 & 2.51 & 0.54 & 12.6 \\

DeFoG{\tiny~\citep{qin2025defog}} $(\eta=0,\omega=0)$
& \small{Flow}
& 200
& 94.6 & 94.6 & 94.1 & 93.8 & 62.7
& 89.6 & 100.0 & 94.7 & 98.6 & 1.93 & 0.55 & 12.8 \\
DeFoG{\tiny~\citep{qin2025defog}} $(\eta=0,\omega=0)$
& \small{Flow}
& 500
& 96.1 & 96.1 & 95.5 & 94.1 & 71.9
& 89.4 & 100.0 & 94.9 & 98.6 & 1.660 & 0.553 & 13.3  \\

\midrule

DeFoG{\tiny~\citep{qin2025defog}}
& \small{Flow}
& 50
& 88.2 & 88.2 & 87.5 & 92.6 & 60.1
& 82.9 & \underline{99.9} & 95.1 & 97.8
& 1.47 & 0.53 & \textbf{19.8} \\

DeFoG{\tiny~\citep{qin2025defog}}
& \small{Flow}
& 100
& 96.7 & 96.7 & 95.7 & 96.0 & 74.2
& 88.5 & 99.9 & 90.7 & 99.2 & 1.25 & 0.58 & 16.7 \\

DeFoG{\tiny~\citep{qin2025defog}}
& \small{Flow}
& 200
& 98.0 & 98.0 & 96.9 & 98.3 & 70.1
& 90.9 & 99.9 & 89.7 & 99.3 & 1.37 & 0.58 & 11.9 \\

DeFoG{\tiny~\citep{qin2025defog}}
& \small{Flow}
& 500
& 98.6 & 98.6 & 97.5 & \textbf{97.6} & 72.5
& \textbf{91.5} & \underline{99.9} & 90.0 & 99.2
& 1.39 & 0.55 & 11.5 \\

\midrule

\rowcolor{gray!15}
\textbf{\ours{}-{DeFoG}(Ours)}
& \small{Flow}
& 50
\\

\rowcolor{gray!15}
\textbf{\ours{}-{DeFoG} (Ours)}
& \small{Flow}
& 100

\\

\rowcolor{gray!15}
\textbf{\ours{}-{DeFoG} (Ours)}
& \small{Flow}
& 200
\\

\rowcolor{gray!15}
\textbf{\ours{}-{DeFoG} (Ours)}
& \small{Flow}
& 500

\\

\midrule

\rowcolor{gray!15}
\textbf{\ours{} (Ours)}
& \small{Flow}
& 50
 \\

\rowcolor{gray!15}
\textbf{\ours{} (Ours)}
& \small{Flow}
& 100
 \\

\rowcolor{gray!15}
\textbf{\ours{} (Ours)}
& \small{Flow}
& 200
 \\

\rowcolor{gray!15}
\textbf{\ours{} (Ours)}
& \small{Flow}
& 500
 \\
\bottomrule
\end{tabular}%
}
\end{table}

==> tables/schedulers_effect.tex <==
\begin{wraptable}{r}{0.35\textwidth}
\vspace{-1\baselineskip}
\centering
\caption{Clock ablations on Planar.}
\vspace{-1em}
\label{tab:planar_clock_ablation}
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.1}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lcc|cc}
\toprule
& \multicolumn{2}{c}{$T=50$}
& \multicolumn{2}{c}{$T=100$} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}
Clock
& VUN $\uparrow$ & Ratio $\downarrow$
& VUN $\uparrow$ & Ratio $\downarrow$ \\
\midrule
\textbf{Hazard-guided (Ours)}
& 99.0 & \textbf{1.83}
& 99.0 & \textbf{1.81} \\
\midrule
Uniform
& 99.5 & 23.43
& \textbf{100.0} & 49.11 \\
Polydec-2
& \textbf{100.0} & 20.20
& \textbf{100.0} & 42.62 \\
Polydec-10
& 99.5 & 5.57
& 99.5 & 12.66 \\
Polydec-20
& 95.5 & 3.88
& 99.5 & 6.08 \\
\bottomrule
\end{tabular}%
}
\vspace{-1.5em}
\end{wraptable}
